Greening File Distribution: Centralized or Distributed?

Despite file-distribution applications are responsible for a major portion of the current Internet traffic, so far little effort has been dedicated to study file distribution from the point of view of energy efficiency. In this paper, we present a first approach at the problem of energy efficiency for file distribution. Specifically, we first demonstrate that the general problem of minimizing energy consumption in file distribution in heterogeneous settings is NP-hard. For homogeneous settings, we derive tight lower bounds on energy consumption, and we design a family of algorithms that achieve these bounds. Our results prove that collaborative p2p schemes achieve up to 50% energy savings with respect to the best available centralized file distribution scheme. Through simulation, we demonstrate that in more realistic cases (e.g., considering network congestion, and link variability across hosts) we validate this observation, since our collaborative algorithms always achieve significant energy savings with respect to the power consumption of centralized file distribution systems.

==> abstract_gianluca.tex <==
\begin{abstract}
%The Internet is growing very rapidly. With it, the total energy consumption of the devices required to keep it functioning properly to meet the demand. While a tremendous amount of research has been done to reduce the energy consumption of the devices, this paper focuses on file distribution mechanism from an energy point of view. We model and characterize the energy consumed in the file distribution from one host to several clients. We derive lower bounds on the energy required for distribution and subsequently design algorithms that achieve these lower bounds proving that upto 50\% energy savings are possible in the best case. Moreover, our scheme are efficient with respect to the time required to finish the process. In addition to the theoretical results, we also discuss some potential scenarios where our schemes can be applied in practice. \\
Despite file-distribution applications are responsible for a major portion of the current Internet traffic, so far little effort has been dedicated to study file distribution from the point of view of energy efficiency. In this paper we present the first deep general study in the field of energy efficiency for file sharing. Specifically, we first demonstrate that the general problem of minimizing energy consumption in file distribution in heterogeneous settings is NP-hard. 
%For a Hence, we analyze restricted versions of the problem, yet maintaining a balance between simplicity and applicability in real networks. 
For homogeneous settings, we derive tight lower bounds on energy consumption, and we design a family of algorithms that achieve these bounds. Our results prove that collaborative p2p schemes achieve up to $50\%$ energy savings with respect to the best available centralized file distribution systems. Through simulation, we demonstrate that in more realistic cases (e.g. considering network congestion) our collaborative algorithms achieve significant energy savings with respect to the power consumption of centralized file distribution systems.

\end{abstract}

==> np-hard.tex <==
\subsection{NP-hardness}
\label{sec:np-hard}

We show in the section that a general version of the problem considered in this paper is NP-hard. 
%In this version of the problem, hosts have different upload and download capacities, different power consumptions, and different block sizes. 
The following theorem summarizes the result.

\begin{thm}
Assume that time is slotted, that hosts must upload at their full capacity, and that no host can upload to more than one host in the same slot.
The problem of minimizing the energy of file distribution is NP-hard if hosts can have different upload capacities and power consumptions, even if
$\alpha_i=\delta_i=0, \forall i$.
\end{thm}
\begin{proof}
We use reduction from the partition problem. 
The input of this problem is a set of integers (we assume all of them to be positive) $A=\{x_0, x_2, ..., x_{k-1}\}$, $k >1$. Let $M=\sum_{x_i \in A} x_i$ to be even. The problem is to decide whether there is a subset $A' \subset A$ such that $\sum_{x_i \in A'} x_i=M/2$.


We reduce an instance of the partition problem to an instance of our problem as follows. The file to distribute has $M$ blocks of size $1$.
There are $n=k+3$ hosts, server $S$, hosts $T$ and $R$, and hosts $H_i$, for $i \in [0,k-1]$.
All hosts have fixed setup energy $\delta_i=0$ and no cost for switching on and off, i.e., $\alpha_i=0$.
Server $S$ has upload capacity $M$ and power $P$.
Host $T$ has download and upload capacity $M$, and power $P$.
Hosts $H_i$, $i \in [0,k-1]$, have download capacity $M$, upload capacity $u_i=x_i$, and power consumption $P$.
Host $R$ has download capacity $M/2$ and power consumption $P' >2P(2k+1)$.
The slot length is one unit of time.

Observe that there is always a feasible solution that respects the assumptions of the model. It works as follows.
First, $S$ serves the whole file to $T$ in one slot. 
Then, $T$ serves the whole file to hosts $H_i$, $i \in [0,k-1]$, in consecutive slots.
Finally, each host $H_i$, $i \in [0,k-1]$, serves $x_i$ different blocks to $R$ in consecutive slots.

We claim that the subset $A'$ that satisfies $\sum_{x_i \in A'} x_i=M/2$ exists if and only if the file distribution problem can be solved with energy smaller than
$3P'$. Hence, the energy minimization problem is NP-hard.

If subset $A'$ exists, the following schedule is feasible.
First, $S$ serves $T$ the whole file in one slot. 
Then, $T$ serves each host $H_i$, $i \in [0,k-1]$, the whole file in consecutive slots.
Let $U=\cup_{x_i \in A'} \{H_i\}$, then the hosts in $U$ upload the file to $R$ in two slots, half the file in each slot.
The total energy consumed is 
$$
E=2P+2Pk+2(|A'|P + P') \leq 2P(2k+1)+2P'<3P'.
$$

Assume now that there is a schedule with energy less than $3P'$. Then, $R$ has been up two slots. Since
they cannot upload at full capacity to $R$, and they cannot serve more than one host, neither $S$ nor $T$ can serve $R$. 
Then, looking at the first slot in which $R$ is up, $R$ must have been served by a subset of hosts $H_i$ whose aggregate 
upload capacity is exactly $M/2$. This proves the existence of $A'$.
\end{proof}
